Finer Behavioral Foundation Models via Auto-Regressive Features and Advantage Weighting

The forward-backward representation (FB) is a recently proposed framework (Touati et al., 2023; Touati & Ollivier, 2021) to train behavior foundation models (BFMs) that aim at providing zero-shot efficient policies for any new task specified in a given reinforcement learning (RL) environment, without training for each new task. Here we address two core limitations of FB model training. First, FB, like all successor-feature-based methods, relies on a linear encoding of tasks: at test time, each new reward function is linearly projected onto a fixed set of pre-trained features. This limits expressivity as well as precision of the task representation. We break the linearity limitation by introducing auto-regressive features for FB, which let finegrained task features depend on coarser-grained task information. This can represent arbitrary nonlinear task encodings, thus significantly increasing expressivity of the FB framework. Second, it is well-known that training RL agents from offline datasets often requires specific techniques.We show that FB works well together with such offline RL techniques, by adapting techniques from (Nair et al.,2020b; Cetin et al., 2024) for FB. This is necessary to get non-flatlining performance in some datasets, such as DMC Humanoid. As a result, we produce efficient FB BFMs for a number of new environments. Notably, in the D4RL locomotion benchmark, the generic FB agent matches the performance of standard single-task offline agents (IQL, XQL). In many setups, the offline techniques are needed to get any decent performance at all. The auto-regressive features have a positive but moderate impact, concentrated on tasks requiring spatial precision and task generalization beyond the behaviors represented in the trainset.

==> 5Results.tex <==

\section{Evaluation}

\subsection{Extended MOOD}






main evaluation based on the MOOD dataset. One concern, is that given that the data in MOOD has been collected with agents trained on the same downstream objectives, all its original tasks maintain a notable present... EDIT
Hence, to evaluate the ability of our new model to generalize beyond this original set, we design additional test tasks for each environment from MOOD





\subsection{D4RL}

\begin{table}[t]

\caption{Performance on the popular locomotion-v2 datasets from the D4RL benchmark, comparing with recent state-of-the-art offline algorithms. FB-AWARE uses 8 AR groups. \edo{other hyper-parameters are tuned per-environment consistently with the offline baselines}}.
\vspace{10pt}
\centering
\adjustbox{max width=0.9\linewidth}{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
Dataset/Algorithm                       & BC    & 10\%BC & DT    & 1StepRL & AWAC  & TD3+BC & CQL   & IQL   & XQL   & ASAC  & FB-AW               & FB-AWARE           \\ \midrule
                                        & \multicolumn{10}{c}{Reward-based learning}                                        & \multicolumn{2}{c}{Reward free learning} \\ \cmidrule(l){2-13} 
halfcheetah-medium-v2                   & 42.6  & 42.5   & 42.6  & 48.4    & 43.5  & 48.3   & 44.0  & 47.4  & 48.3  & 61.6  & 60.0±0.9            & 62.7±0.9           \\
hopper-medium-v2                        & 52.9  & 56.9   & 67.6  & 59.6    & 57.0  & 59.3   & 58.5  & 66.3  & 74.2  & 94.3  & 59.1±5.0            & 59.9±21.4          \\
walker2d-medium-v2                      & 75.3  & 75.0   & 74.0  & 81.8    & 72.4  & 83.7   & 72.5  & 78.3  & 84.2  & 89.1  & 80.5±11.7           & 89.6±0.8           \\
halfcheetah-medium-replay-v2            & 36.6  & 40.6   & 36.6  & 38.1    & 40.5  & 44.6   & 45.5  & 44.2  & 45.2  & 55.2  & 52.7±1.2            & 50.8±1.2           \\
hopper-medium-replay-v2                 & 18.1  & 75.9   & 82.7  & 97.5    & 37.2  & 60.9   & 95.0  & 94.7  & 100.7 & 101.5 & 87.1±3.7            & 89.6±4.0           \\
walker2d-medium-replay-v2               & 26.0  & 62.5   & 66.6  & 49.5    & 27.0  & 81.8   & 77.2  & 73.9  & 82.2  & 91.4  & 91.7±6.3            & 98.8±0.5           \\
halfcheetah-medium-expert-v2            & 55.2  & 92.9   & 86.8  & 93.4    & 42.8  & 90.7   & 91.6  & 86.7  & 94.2  & 96.0  & 99.6±0.8            & 100.1±0.7          \\
hopper-medium-expert-v2                 & 52.5  & 110.9  & 107.6 & 103.3   & 55.8  & 98.0   & 105.4 & 91.5  & 111.2 & 111.9 & 55.9±11.6           & 62.2±9.2           \\
walker2d-medium-expert-v2               & 107.5 & 109.0  & 108.1 & 113.0   & 74.5  & 110.1  & 108.8 & 109.6 & 112.7 & 113.9 & 109.6±1.3           & 105.8±0.6          \\
\multicolumn{1}{c}{Locomotion-v2 total} & 466.7 & 666.2  & 672.6 & 684.6   & 450.7 & 677.4  & 698.5 & 692.6 & 752.9 & 815.9 & 696.2               & 719.5              \\ \bottomrule
\end{tabular}

}
\end{table}


Finally, to test the generality and robustness of our methods, we test
its performance on the D4RL benchmark after reward-free training.
Here, we are comparing the multitask, unsupervised FB-AWARE agent to
task-specifics agents, sot he performance of the latter are a natural
topline for FB-AWARE. In line with \cite{fb_0shot}, we expect FB-AWARE to
reach a good fraction of the performance of the agents trained specifically on
each task.

So we compare FB-AWARE's performance with the results available for a
large pool of offline RL algorithms optimizing for an individual
objective with full access to rewards. We note this setting is quite
different in nature than... , since D4RL datasets mostly comprise
trajectories from agents trying to accomplish a single...




==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\deq}{\mathrel{\mathop{:}}=}
\newcommand{\eqd}{=\mathrel{\mathop{:}}}


\newcommand{\calB}{\mathcal{B}}


==> tables_store.tex <==


\begin{tabular}{lllllll}
\hline
 Domain    & Task          & fb\_or\_fp           & fb\_fp              & fbiw\_abl\_nofp\_min   & fbiw\_abl\_awac      & fb\_aw              \\
\hline
 cheetah   & walk          & 275.5\tiny{±343.5} & 500.2\tiny{±285.2} & 987.5\tiny{±0.6}    & 975.0\tiny{±23.5}  & 975.6\tiny{±24.6}  \\
 cheetah   & run           & 77.1\tiny{±87.3}   & 106.0\tiny{±50.4}  & 548.3\tiny{±38.6}   & 548.4\tiny{±30.0}  & 610.7\tiny{±49.2}  \\
 cheetah   & walk\_backward & 199.3\tiny{±209.1} & 349.7\tiny{±394.5} & 984.8\tiny{±0.4}    & 984.5\tiny{±1.2}   & 984.7\tiny{±0.4}   \\
 cheetah   & run\_backward  & 49.1\tiny{±58.6}   & 78.6\tiny{±118.3}  & 461.0\tiny{±6.6}    & 477.4\tiny{±7.8}   & 481.4\tiny{±4.2}   \\
 cheetah   & train\_avg     & 0.175\tiny{±0.203} & 0.295\tiny{±0.249} & 0.939\tiny{±0.019}  & 0.944\tiny{±0.022} & 0.971\tiny{±0.028} \\
 quadruped & walk          & 318.3\tiny{±65.7}  & 763.9\tiny{±145.2} & 889.4\tiny{±80.5}   & 938.8\tiny{±34.7}  & 958.0\tiny{±9.1}   \\
 quadruped & run           & 279.4\tiny{±45.8}  & 439.8\tiny{±90.2}  & 446.1\tiny{±50.6}   & 599.4\tiny{±70.4}  & 673.4\tiny{±33.1}  \\
 quadruped & stand         & 619.6\tiny{±121.1} & 831.5\tiny{±147.8} & 901.3\tiny{±84.7}   & 944.9\tiny{±44.0}  & 975.9\tiny{±4.5}   \\
 quadruped & jump          & 435.0\tiny{±79.8}  & 644.1\tiny{±127.7} & 708.2\tiny{±20.2}   & 767.4\tiny{±74.9}  & 798.4\tiny{±55.0}  \\
 quadruped & train\_avg     & 0.493\tiny{±0.093} & 0.800\tiny{±0.153} & 0.877\tiny{±0.070}  & 0.976\tiny{±0.070} & 1.026\tiny{±0.032} \\
 walker    & stand         & 906.5\tiny{±80.4}  & 976.2\tiny{±9.5}   & 964.8\tiny{±3.5}    & 978.9\tiny{±3.1}   & 956.1\tiny{±34.7}  \\
 walker    & walk          & 892.8\tiny{±102.7} & 939.9\tiny{±44.7}  & 946.7\tiny{±10.3}   & 960.1\tiny{±7.3}   & 955.4\tiny{±16.6}  \\
 walker    & run           & 462.2\tiny{±37.5}  & 487.0\tiny{±44.1}  & 480.5\tiny{±52.6}   & 583.3\tiny{±20.9}  & 579.8\tiny{±45.8}  \\
 walker    & spin          & 422.1\tiny{±121.4} & 464.9\tiny{±196.4} & 923.2\tiny{±30.1}   & 759.2\tiny{±173.6} & 789.6\tiny{±117.7} \\
 walker    & train\_avg     & 0.749\tiny{±0.093} & 0.799\tiny{±0.081} & 0.913\tiny{±0.032}  & 0.918\tiny{±0.055} & 0.917\tiny{±0.061} \\
 humanoid  & walk          & 3.6\tiny{±5.0}     & 2.3\tiny{±1.1}     & 677.6\tiny{±52.8}   & 779.9\tiny{±37.1}  & 785.0\tiny{±20.4}  \\
 humanoid  & stand         & 5.1\tiny{±1.9}     & 4.8\tiny{±0.8}     & 481.3\tiny{±59.5}   & 750.3\tiny{±43.3}  & 801.7\tiny{±45.8}  \\
 humanoid  & run           & 1.1\tiny{±0.8}     & 1.1\tiny{±0.6}     & 256.8\tiny{±22.9}   & 274.4\tiny{±20.4}  & 294.9\tiny{±17.5}  \\
 humanoid  & train\_avg     & 0.005\tiny{±0.004} & 0.004\tiny{±0.002} & 0.793\tiny{±0.074}  & 0.965\tiny{±0.058} & 1.014\tiny{±0.049} \\
 cheetah   & bounce        & 109.6\tiny{±83.9}  & 315.4\tiny{±102.8} & 436.3\tiny{±47.1}   & 469.3\tiny{±39.7}  & 502.5\tiny{±19.2}  \\
 cheetah   & march         & 135.8\tiny{±182.5} & 257.8\tiny{±110.2} & 766.9\tiny{±92.7}   & 892.6\tiny{±35.0}  & 917.4\tiny{±13.4}  \\
 cheetah   & stand         & 206.6\tiny{±383.7} & 684.7\tiny{±267.4} & 426.9\tiny{±191.6}  & 288.9\tiny{±162.6} & 387.6\tiny{±98.4}  \\
 cheetah   & headstand     & 233.8\tiny{±369.0} & 923.7\tiny{±57.1}  & 488.0\tiny{±345.1}  & 407.0\tiny{±369.8} & 854.5\tiny{±42.0}  \\
 cheetah   & test\_avg      & 0.214\tiny{±0.308} & 0.684\tiny{±0.166} & 0.660\tiny{±0.207}  & 0.642\tiny{±0.188} & 0.832\tiny{±0.053} \\
 quadruped & bounce        & 133.6\tiny{±82.8}  & 248.9\tiny{±41.0}  & 204.3\tiny{±61.0}   & 246.6\tiny{±31.3}  & 231.8\tiny{±18.4}  \\
 quadruped & skip          & 478.9\tiny{±113.2} & 601.0\tiny{±72.3}  & 554.0\tiny{±1.3}    & 722.7\tiny{±112.4} & 836.1\tiny{±104.4} \\
 quadruped & march         & 280.8\tiny{±73.1}  & 517.2\tiny{±108.0} & 478.8\tiny{±41.8}   & 802.1\tiny{±55.9}  & 860.2\tiny{±26.7}  \\
 quadruped & trot          & 178.3\tiny{±38.0}  & 381.5\tiny{±82.6}  & 412.1\tiny{±48.6}   & 605.3\tiny{±16.9}  & 615.9\tiny{±13.6}  \\
 quadruped & test\_avg      & 0.524\tiny{±0.175} & 0.897\tiny{±0.159} & 0.834\tiny{±0.105}  & 1.187\tiny{±0.105} & 1.245\tiny{±0.075} \\
 walker    & flip          & 630.3\tiny{±111.7} & 744.4\tiny{±105.4} & 771.8\tiny{±104.5}  & 891.2\tiny{±24.9}  & 896.5\tiny{±41.2}  \\
 walker    & march         & 709.4\tiny{±182.1} & 744.6\tiny{±183.3} & 593.9\tiny{±12.6}   & 788.3\tiny{±63.7}  & 797.2\tiny{±36.8}  \\
 walker    & skyreach      & 321.7\tiny{±130.0} & 423.0\tiny{±70.3}  & 392.7\tiny{±15.1}   & 364.3\tiny{±48.0}  & 389.8\tiny{±6.5}   \\
 walker    & pullup        & 114.7\tiny{±98.5}  & 101.3\tiny{±104.1} & 33.9\tiny{±8.2}     & 309.7\tiny{±145.5} & 376.5\tiny{±219.5} \\
 walker    & test\_avg      & 0.645\tiny{±0.196} & 0.747\tiny{±0.163} & 0.674\tiny{±0.052}  & 0.849\tiny{±0.101} & 0.889\tiny{±0.101} \\
 humanoid  & dive          & 159.2\tiny{±12.2}  & 166.6\tiny{±29.5}  & 357.1\tiny{±36.6}   & 387.9\tiny{±39.8}  & 404.0\tiny{±5.7}   \\
 humanoid  & march         & 2.9\tiny{±3.5}     & 2.9\tiny{±1.8}     & 479.6\tiny{±48.5}   & 623.1\tiny{±64.6}  & 645.9\tiny{±49.7}  \\
 humanoid  & skip          & 2.0\tiny{±1.2}     & 1.7\tiny{±0.4}     & 81.3\tiny{±26.7}    & 254.4\tiny{±23.8}  & 250.1\tiny{±24.0}  \\
 humanoid  & test\_avg      & 0.112\tiny{±0.011} & 0.117\tiny{±0.021} & 0.536\tiny{±0.072}  & 0.788\tiny{±0.079} & 0.805\tiny{±0.049} \\
\hline
\end{tabular}








\begin{tabular}{llllll}
\hline
 Domain   & Task               & fb\_aw\_rnd          & fb\_aw\_mood         & fb\_aw\_8ar\_rnd      & fb\_aw\_8ar\_mood     \\
\hline
 jaco     & reach\_top\_left     & 51.6\tiny{±14.5}   & 121.0\tiny{±11.0}  & 81.2\tiny{±7.2}    & 97.9\tiny{±17.8}   \\
 jaco     & reach\_top\_right    & 62.4\tiny{±22.0}   & 125.0\tiny{±31.4}  & 72.3\tiny{±29.0}   & 145.3\tiny{±28.7}  \\
 jaco     & reach\_bottom\_left  & 49.0\tiny{±27.4}   & 140.8\tiny{±29.5}  & 99.0\tiny{±33.2}   & 147.0\tiny{±29.6}  \\
 jaco     & reach\_bottom\_right & 64.9\tiny{±23.7}   & 99.0\tiny{±39.1}   & 95.7\tiny{±46.6}   & 155.6\tiny{±23.1}  \\
 jaco     & train\_avg          & 0.402\tiny{±0.153} & 0.864\tiny{±0.190} & 0.614\tiny{±0.196} & 0.952\tiny{±0.174} \\
 jaco     & reach\_random1      & 60.8\tiny{±19.9}   & 39.5\tiny{±15.8}   & 54.9\tiny{±22.6}   & 55.2\tiny{±23.1}   \\
 jaco     & reach\_random2      & 56.9\tiny{±22.5}   & 35.6\tiny{±15.5}   & 112.5\tiny{±32.3}  & 45.7\tiny{±11.1}   \\
 jaco     & reach\_random3      & 49.4\tiny{±13.9}   & 30.1\tiny{±13.9}   & 52.3\tiny{±29.7}   & 30.4\tiny{±21.4}   \\
 jaco     & reach\_random4      & 43.5\tiny{±23.2}   & 53.1\tiny{±9.4}    & 102.8\tiny{±41.9}  & 70.5\tiny{±29.7}   \\
 jaco     & test\_avg           & 0.718\tiny{±0.254} & 0.515\tiny{±0.189} & 0.976\tiny{±0.408} & 0.645\tiny{±0.294} \\
\hline
\end{tabular}






\begin{tabular}{llllll}
\hline
 Domain    & Task          & fb\_or\_fp           & fb\_aw              & fb\_aw\_4ar          & fb\_aw\_8ar          \\
\hline
 cheetah   & walk          & 275.5\tiny{±343.5} & 975.6\tiny{±24.6}  & 972.5\tiny{±18.0}  & 984.1\tiny{±3.1}   \\
 cheetah   & run           & 77.1\tiny{±87.3}   & 610.7\tiny{±49.2}  & 586.7\tiny{±36.3}  & 586.2\tiny{±28.8}  \\
 cheetah   & walk\_backward & 199.3\tiny{±209.1} & 984.7\tiny{±0.4}   & 983.3\tiny{±0.8}   & 982.6\tiny{±5.4}   \\
 cheetah   & run\_backward  & 49.1\tiny{±58.6}   & 481.4\tiny{±4.2}   & 502.0\tiny{±18.5}  & 506.9\tiny{±12.5}  \\
 cheetah   & train\_avg     & 0.175\tiny{±0.203} & 0.971\tiny{±0.028} & 0.970\tiny{±0.028} & 0.975\tiny{±0.020} \\
 quadruped & walk          & 318.3\tiny{±65.7}  & 958.0\tiny{±9.1}   & 962.8\tiny{±12.9}  & 958.7\tiny{±10.7}  \\
 quadruped & run           & 279.4\tiny{±45.8}  & 673.4\tiny{±33.1}  & 663.1\tiny{±37.2}  & 611.8\tiny{±39.6}  \\
 quadruped & stand         & 619.6\tiny{±121.1} & 975.9\tiny{±4.5}   & 976.2\tiny{±2.9}   & 974.2\tiny{±6.0}   \\
 quadruped & jump          & 435.0\tiny{±79.8}  & 798.4\tiny{±55.0}  & 870.9\tiny{±9.9}   & 766.3\tiny{±85.3}  \\
 quadruped & train\_avg     & 0.493\tiny{±0.093} & 1.026\tiny{±0.032} & 1.046\tiny{±0.021} & 0.994\tiny{±0.045} \\
 walker    & stand         & 906.5\tiny{±80.4}  & 956.1\tiny{±34.7}  & 972.8\tiny{±9.1}   & 970.9\tiny{±12.0}  \\
 walker    & walk          & 892.8\tiny{±102.7} & 955.4\tiny{±16.6}  & 943.3\tiny{±9.1}   & 925.6\tiny{±13.9}  \\
 walker    & run           & 462.2\tiny{±37.5}  & 579.8\tiny{±45.8}  & 650.8\tiny{±6.8}   & 646.3\tiny{±41.0}  \\
 walker    & spin          & 422.1\tiny{±121.4} & 789.6\tiny{±117.7} & 759.5\tiny{±149.0} & 937.4\tiny{±69.8}  \\
 walker    & train\_avg     & 0.749\tiny{±0.093} & 0.917\tiny{±0.061} & 0.938\tiny{±0.046} & 0.977\tiny{±0.040} \\
 humanoid  & walk          & 3.6\tiny{±5.0}     & 785.0\tiny{±20.4}  & 782.8\tiny{±40.1}  & 772.8\tiny{±16.1}  \\
 humanoid  & stand         & 5.1\tiny{±1.9}     & 801.7\tiny{±45.8}  & 679.7\tiny{±7.2}   & 720.4\tiny{±81.3}  \\
 humanoid  & run           & 1.1\tiny{±0.8}     & 294.9\tiny{±17.5}  & 311.3\tiny{±18.2}  & 305.3\tiny{±15.8}  \\
 humanoid  & train\_avg     & 0.005\tiny{±0.004} & 1.014\tiny{±0.049} & 0.984\tiny{±0.042} & 0.989\tiny{±0.059} \\
 cheetah   & bounce        & 109.6\tiny{±83.9}  & 502.5\tiny{±19.2}  & 553.3\tiny{±20.2}  & 544.2\tiny{±5.4}   \\
 cheetah   & march         & 135.8\tiny{±182.5} & 917.4\tiny{±13.4}  & 962.4\tiny{±23.6}  & 940.5\tiny{±62.8}  \\
 cheetah   & stand         & 206.6\tiny{±383.7} & 387.6\tiny{±98.4}  & 561.8\tiny{±91.6}  & 635.1\tiny{±133.9} \\
 cheetah   & headstand     & 233.8\tiny{±369.0} & 854.5\tiny{±42.0}  & 860.4\tiny{±114.3} & 894.3\tiny{±37.0}  \\
 cheetah   & test\_avg      & 0.214\tiny{±0.308} & 0.832\tiny{±0.053} & 0.916\tiny{±0.077} & 0.938\tiny{±0.069} \\
 quadruped & bounce        & 133.6\tiny{±82.8}  & 231.8\tiny{±18.4}  & 343.3\tiny{±28.7}  & 287.6\tiny{±24.2}  \\
 quadruped & skip          & 478.9\tiny{±113.2} & 836.1\tiny{±104.4} & 933.5\tiny{±58.0}  & 789.2\tiny{±98.6}  \\
 quadruped & march         & 280.8\tiny{±73.1}  & 860.2\tiny{±26.7}  & 874.4\tiny{±22.7}  & 878.1\tiny{±33.6}  \\
 quadruped & trot          & 178.3\tiny{±38.0}  & 615.9\tiny{±13.6}  & 693.3\tiny{±18.8}  & 680.2\tiny{±12.6}  \\
 quadruped & test\_avg      & 0.524\tiny{±0.175} & 1.245\tiny{±0.075} & 1.436\tiny{±0.069} & 1.325\tiny{±0.081} \\
 walker    & flip          & 630.3\tiny{±111.7} & 896.5\tiny{±41.2}  & 978.0\tiny{±7.2}   & 975.5\tiny{±18.7}  \\
 walker    & march         & 709.4\tiny{±182.1} & 797.2\tiny{±36.8}  & 897.9\tiny{±34.6}  & 863.0\tiny{±22.5}  \\
 walker    & skyreach      & 321.7\tiny{±130.0} & 389.8\tiny{±6.5}   & 392.5\tiny{±16.6}  & 473.0\tiny{±49.0}  \\
 walker    & pullup        & 114.7\tiny{±98.5}  & 376.5\tiny{±219.5} & 561.9\tiny{±53.9}  & 554.2\tiny{±51.9}  \\
 walker    & test\_avg      & 0.645\tiny{±0.196} & 0.889\tiny{±0.101} & 1.011\tiny{±0.039} & 1.041\tiny{±0.057} \\
 humanoid  & dive          & 159.2\tiny{±12.2}  & 404.0\tiny{±5.7}   & 473.9\tiny{±68.6}  & 451.1\tiny{±43.8}  \\
 humanoid  & march         & 2.9\tiny{±3.5}     & 645.9\tiny{±49.7}  & 728.9\tiny{±88.2}  & 680.3\tiny{±54.2}  \\
 humanoid  & skip          & 2.0\tiny{±1.2}     & 250.1\tiny{±24.0}  & 295.6\tiny{±40.7}  & 297.9\tiny{±20.4}  \\
 humanoid  & test\_avg      & 0.112\tiny{±0.011} & 0.805\tiny{±0.049} & 0.934\tiny{±0.125} & 0.899\tiny{±0.074} \\
\hline
\end{tabular}




\begin{table}[H]
    \centering
\begin{tabular}{llllll}
\hline
 Domain    & Task          & fb\_or\_fp           & fb\_aw              & fb\_aw\_4ar          & fb\_aw\_8ar          \\
\hline
 cheetah   & walk          & 811.1\tiny{±95.8}  & 968.7\tiny{±9.8}   & 890.8\tiny{±61.3}  & 880.7\tiny{±101.1} \\
 cheetah   & run           & 266.4\tiny{±40.1}  & 332.4\tiny{±23.2}  & 257.3\tiny{±59.1}  & 271.3\tiny{±49.4}  \\
 cheetah   & walk\_backward & 849.0\tiny{±193.0} & 978.1\tiny{±8.8}   & 947.0\tiny{±36.9}  & 946.6\tiny{±34.9}  \\
 cheetah   & run\_backward  & 218.2\tiny{±71.0}  & 269.4\tiny{±37.6}  & 219.8\tiny{±23.9}  & 220.7\tiny{±23.9}  \\
 cheetah   & train\_avg     & 0.631\tiny{±0.123} & 0.755\tiny{±0.032} & 0.673\tiny{±0.060} & 0.677\tiny{±0.066} \\
 quadruped & walk          & 694.2\tiny{±135.5} & 430.7\tiny{±28.1}  & 502.0\tiny{±6.0}   & 504.9\tiny{±8.4}   \\
 quadruped & run           & 507.6\tiny{±16.5}  & 431.2\tiny{±26.8}  & 488.5\tiny{±1.2}   & 487.0\tiny{±3.9}   \\
 quadruped & stand         & 979.0\tiny{±5.1}   & 849.1\tiny{±61.0}  & 972.7\tiny{±4.2}   & 974.1\tiny{±5.1}   \\
 quadruped & jump          & 811.8\tiny{±20.2}  & 623.9\tiny{±40.0}  & 798.6\tiny{±8.0}   & 797.7\tiny{±5.3}   \\
 quadruped & train\_avg     & 0.896\tiny{±0.052} & 0.700\tiny{±0.047} & 0.828\tiny{±0.006} & 0.829\tiny{±0.007} \\
 walker    & stand         & 818.6\tiny{±75.8}  & 674.1\tiny{±92.2}  & 636.0\tiny{±40.8}  & 634.5\tiny{±38.4}  \\
 walker    & walk          & 777.6\tiny{±71.6}  & 680.6\tiny{±57.8}  & 633.5\tiny{±31.4}  & 632.5\tiny{±32.1}  \\
 walker    & run           & 393.2\tiny{±41.7}  & 353.1\tiny{±36.5}  & 313.0\tiny{±17.0}  & 311.1\tiny{±15.9}  \\
 walker    & spin          & 372.4\tiny{±55.3}  & 344.8\tiny{±62.7}  & 245.2\tiny{±88.5}  & 250.2\tiny{±88.8}  \\
 walker    & train\_avg     & 0.657\tiny{±0.068} & 0.573\tiny{±0.069} & 0.510\tiny{±0.048} & 0.510\tiny{±0.047} \\
 cheetah   & bounce        & 352.6\tiny{±37.2}  & 327.7\tiny{±87.5}  & 239.3\tiny{±162.6} & 227.6\tiny{±168.0} \\
 cheetah   & march         & 539.2\tiny{±91.3}  & 641.8\tiny{±30.2}  & 512.7\tiny{±88.1}  & 506.9\tiny{±99.8}  \\
 cheetah   & stand         & 102.6\tiny{±50.3}  & 69.5\tiny{±78.4}   & 15.7\tiny{±30.3}   & 10.9\tiny{±21.2}   \\
 cheetah   & headstand     & 947.6\tiny{±9.3}   & 954.6\tiny{±5.0}   & 886.4\tiny{±88.4}  & 896.6\tiny{±75.8}  \\
 cheetah   & test\_avg      & 0.617\tiny{±0.057} & 0.627\tiny{±0.068} & 0.519\tiny{±0.127} & 0.515\tiny{±0.126} \\
 quadruped & bounce        & 271.2\tiny{±78.9}  & 42.8\tiny{±19.0}   & 70.3\tiny{±9.0}    & 91.3\tiny{±14.2}   \\
 quadruped & skip          & 676.9\tiny{±28.5}  & 490.5\tiny{±48.6}  & 587.3\tiny{±13.3}  & 602.1\tiny{±10.9}  \\
 quadruped & march         & 530.6\tiny{±35.4}  & 427.7\tiny{±32.2}  & 491.0\tiny{±1.7}   & 490.2\tiny{±4.1}   \\
 quadruped & trot          & 400.0\tiny{±37.6}  & 281.1\tiny{±17.5}  & 348.7\tiny{±2.1}   & 346.3\tiny{±6.7}   \\
 quadruped & test\_avg      & 0.962\tiny{±0.124} & 0.561\tiny{±0.060} & 0.687\tiny{±0.015} & 0.711\tiny{±0.023} \\
 walker    & flip          & 445.3\tiny{±54.0}  & 394.9\tiny{±47.2}  & 372.3\tiny{±33.2}  & 374.1\tiny{±34.6}  \\
 walker    & march         & 685.5\tiny{±70.2}  & 568.8\tiny{±71.5}  & 551.5\tiny{±37.3}  & 551.7\tiny{±30.5}  \\
 walker    & skyreach      & 339.3\tiny{±74.2}  & 291.6\tiny{±115.1} & 304.0\tiny{±58.3}  & 307.9\tiny{±49.1}  \\
 walker    & pullup        & 135.0\tiny{±53.0}  & 44.5\tiny{±34.4}   & 44.7\tiny{±26.3}   & 44.3\tiny{±24.8}   \\
 walker    & test\_avg      & 0.587\tiny{±0.097} & 0.480\tiny{±0.111} & 0.473\tiny{±0.063} & 0.476\tiny{±0.056} \\
\hline
\end{tabular}
\caption{\label{tab: rnd resutls} RND results}
\end{table}


\begin{table}[H]
\begin{tabular}{lll}
\hline
 Domain    & Task          & sf\_lap                \\
\hline
 cheetah   & walk          & 987.4\tiny{±1.2}      \\
 cheetah   & run           & 580.5\tiny{±29.9}     \\
 cheetah   & walk\_backward & 986.1\tiny{±0.2}      \\
 cheetah   & run\_backward  & 419.9\tiny{±10.4}     \\
 cheetah   & train\_avg     & 743.473\tiny{±10.439} \\
 quadruped & walk          & 914.6\tiny{±39.7}     \\
 quadruped & run           & 527.4\tiny{±96.9}     \\
 quadruped & stand         & 841.3\tiny{±126.9}    \\
 quadruped & jump          & 702.3\tiny{±42.4}     \\
 quadruped & train\_avg     & 746.404\tiny{±76.448} \\
 walker    & stand         & 923.1\tiny{±34.6}     \\
 walker    & walk          & 943.9\tiny{±15.8}     \\
 walker    & run           & 483.2\tiny{±35.9}     \\
 walker    & spin          & 669.8\tiny{±167.6}    \\
 walker    & train\_avg     & 754.992\tiny{±63.487} \\
 humanoid  & walk          & 741.8\tiny{±32.7}     \\
 humanoid  & stand         & 554.3\tiny{±27.0}     \\
 humanoid  & run           & 247.7\tiny{±13.7}     \\
 humanoid  & train\_avg     & 514.597\tiny{±24.466} \\
 cheetah   & bounce        & 230.4\tiny{±27.4}     \\
 cheetah   & march         & 859.1\tiny{±39.4}     \\
 cheetah   & stand         & 194.5\tiny{±34.9}     \\
 cheetah   & headstand     & 0.0\tiny{±0.0}        \\
 cheetah   & test\_avg      & 321.022\tiny{±25.436} \\
 quadruped & bounce        & 201.9\tiny{±37.6}     \\
 quadruped & skip          & 723.5\tiny{±118.3}    \\
 quadruped & march         & 706.2\tiny{±101.5}    \\
 quadruped & trot          & 428.0\tiny{±91.5}     \\
 quadruped & test\_avg      & 514.886\tiny{±87.216} \\
 walker    & flip          & 720.2\tiny{±94.5}     \\
 walker    & march         & 815.6\tiny{±57.2}     \\
 walker    & skyreach      & 323.4\tiny{±60.2}     \\
 walker    & pullup        & 65.0\tiny{±18.0}      \\
 walker    & test\_avg      & 481.030\tiny{±57.476} \\
 humanoid  & dive          & 279.3\tiny{±42.1}     \\
 humanoid  & march         & 534.7\tiny{±90.8}     \\
 humanoid  & skip          & 150.7\tiny{±23.0}     \\
 humanoid  & test\_avg      & 321.576\tiny{±51.951} \\
\hline
\end{tabular}
\caption{ laplacian results on MOOD}
\end{table}



\begin{table}[H]
    \centering
    \begin{tabular}{lllll}
\hline
 Domain    & Task          & fb2                    & fb2p                   & arfb-64-4             \\
\hline
 cheetah   & walk          & 926.7\tiny{±92.6}      & 769.0\tiny{±176.5}     & 700.4\tiny{±153.2}    \\
 cheetah   & run           & 327.3\tiny{±42.6}      & 315.0\tiny{±107.5}     & 268.7\tiny{±67.3}     \\
 cheetah   & walk\_backward & 828.2\tiny{±205.8}     & 691.3\tiny{±148.1}     & 855.6\tiny{±127.5}    \\
 cheetah   & run\_backward  & 212.0\tiny{±53.6}      & 162.6\tiny{±36.0}      & 196.5\tiny{±51.6}     \\
 cheetah   & train\_avg     & 573.516\tiny{±98.639}  & 484.448\tiny{±117.049} & 505.321\tiny{±99.891} \\
 quadruped & walk          & 745.1\tiny{±79.1}      & 558.3\tiny{±20.6}      & 710.2\tiny{±110.1}    \\
 quadruped & run           & 470.0\tiny{±58.1}      & 408.2\tiny{±19.2}      & 437.7\tiny{±69.5}     \\
 quadruped & stand         & 871.5\tiny{±111.3}     & 770.9\tiny{±28.4}      & 762.2\tiny{±103.9}    \\
 quadruped & jump          & 664.9\tiny{±121.0}     & 652.5\tiny{±25.5}      & 601.4\tiny{±54.8}     \\
 quadruped & train\_avg     & 687.852\tiny{±92.388}  & 597.452\tiny{±23.429}  & 627.882\tiny{±84.597} \\
 walker    & stand         & 889.6\tiny{±64.3}      & 764.1\tiny{±82.0}      & 731.1\tiny{±137.3}    \\
 walker    & walk          & 878.8\tiny{±45.2}      & 744.8\tiny{±40.3}      & 744.1\tiny{±30.3}     \\
 walker    & run           & 411.8\tiny{±25.8}      & 370.1\tiny{±43.0}      & 404.9\tiny{±27.2}     \\
 walker    & spin          & 978.8\tiny{±8.0}       & 982.6\tiny{±4.2}       & 982.5\tiny{±3.4}      \\
 walker    & train\_avg     & 789.755\tiny{±35.823}  & 715.399\tiny{±42.385}  & 715.651\tiny{±49.556} \\
 cheetah   & bounce        & 496.9\tiny{±160.0}     & 440.4\tiny{±61.1}      & 473.4\tiny{±49.9}     \\
 cheetah   & march         & 653.0\tiny{±74.3}      & 586.3\tiny{±201.1}     & 522.5\tiny{±118.8}    \\
 cheetah   & stand         & 314.5\tiny{±129.5}     & 673.5\tiny{±79.8}      & 803.9\tiny{±45.7}     \\
 cheetah   & headstand     & 640.0\tiny{±335.6}     & 769.9\tiny{±252.1}     & 864.9\tiny{±38.1}     \\
 cheetah   & test\_avg      & 526.106\tiny{±174.845} & 617.516\tiny{±148.536} & 666.191\tiny{±63.127} \\
 quadruped & bounce        & 128.4\tiny{±144.0}     & 278.0\tiny{±52.8}      & 310.2\tiny{±137.3}    \\
 quadruped & skip          & 621.6\tiny{±88.7}      & 652.8\tiny{±34.5}      & 648.7\tiny{±59.5}     \\
 quadruped & march         & 519.6\tiny{±76.3}      & 452.6\tiny{±10.4}      & 527.3\tiny{±68.5}     \\
 quadruped & trot          & 397.9\tiny{±66.2}      & 384.3\tiny{±19.9}      & 402.2\tiny{±54.5}     \\
 quadruped & test\_avg      & 416.856\tiny{±93.798}  & 441.914\tiny{±29.402}  & 472.094\tiny{±79.964} \\
 walker    & flip          & 547.9\tiny{±101.4}     & 440.4\tiny{±159.7}     & 506.6\tiny{±24.1}     \\
 walker    & march         & 712.2\tiny{±70.1}      & 621.8\tiny{±69.1}      & 511.0\tiny{±55.5}     \\
 walker    & skyreach      & 599.0\tiny{±117.0}     & 436.3\tiny{±69.1}      & 358.5\tiny{±31.9}     \\
 walker    & pullup        & 76.5\tiny{±107.7}      & 384.1\tiny{±150.7}     & 404.4\tiny{±76.7}     \\
 walker    & test\_avg      & 483.902\tiny{±99.058}  & 470.626\tiny{±112.181} & 445.149\tiny{±47.079} \\
\hline
\end{tabular}
    \caption{new rnd}
    \label{tab:my_label}
\end{table}



